DeepMapping2: Self-Supervised Large-Scale LiDAR Map Optimization

LiDAR mapping is important yet challenging in self-driving and mobile robotics. To tackle such a global point cloud registration problem, DeepMapping converts the complex map estimation into a self-supervised training of simple deep networks. Despite its broad convergence range on small datasets, DeepMapping still cannot produce satisfactory results on large-scale datasets with thousands of frames. This is due to the lack of loop closures and exact cross-frame point correspondences, and the slow convergence of its global localization network. We propose DeepMapping2 by adding two novel techniques to address these issues: (1) organization of training batch based on map topology from loop closing, and (2) self-supervised local-to-global point consistency loss leveraging pairwise registration. Our experiments and ablation studies on public datasets (KITTI, NCLT, and Nebula) demonstrate the effectiveness of our method.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{balance}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{multirow, multicol}
% \usepackage{makecell}
% \usepackage{wrapfig}
% \usepackage[table,dvipsnames]{xcolor}



% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref,breaklinks,colorlinks,bookmarks=false]{hyperref}
% \input{packages} % For convenient comment

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\cvprPaperID{8635} % *** Enter the CVPR Paper ID here
% \def\confName{CVPR}
% \def\confYear{2023}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{\textit{Rebuttal for} DeepMapping2: Self-Supervised Large-Scale LiDAR Map Optimization
% \vspace{-3mm}
% }  % **** Enter the paper title here

% \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
% We thank reviewers for the appreciation (``well-written'' (Reviewer oReC $\&$ vwoA),  ``the idea is clearly demonstrated'' (Reviewer oReC), and ``the experiment is detailed'' (Reviewer tdMN)) and the constructive feedback. We first address three common concerns and then respond to individual concerns from the reviewers.

% % We sincerely appreciate your constructive feedback. We appreciate the positive comments such as ``well-written'' (Reviewer oReC$\&$Reviewer vwoA), ``the idea is clearly demonstrated'' (Reviewer oReC), ``the previous work is well summarized'', ``good extension'', ``comprehensive evaluation'' (Reviewer vwoA), ``this paper is clear'', and ``the experiment is detailed'' (Reviewer tdMN). We will add more baselines as the reviewers cited and provide more detailed ablation study in our final version.

% % —————————————————————————————————————————————————————————————— 
% % \textbf{Common Concern}
% % \vspace{+1mm}

% %KISS-ICP~\cite{vizzo2023kiss}
% % Baselines and baseline integration with DeepMapping2
% \textbf{Reviewers oReC \& tdMN: Additional comparisons with SOTA.} As suggested, we include a performance comparison against the original \textit{DeepMapping (DM)}, \textit{HRegNet}, and \textit{GeoTransformer}. We also include a recent method, \textit{KISS-ICP}~\footnote{Vizzo et al., ``KISS-ICP: In defense of point-to-point ICP simple, accurate, and robust registration if done the right way,'' IEEE RA-L 2023}.
% The results in \cref{tab:kitti_ate} \textbf{reinforce our findings that \textit{DM2} significantly outperforms\footnote{As well recognized in 3D vision, reducing the Absolute Trajectory Error (ATE), averaged across all frames, for several meters/decimeters (e.g., $6.25\to 2.29$) is non-trivial and significant because even a small trajectory error could mean a large mapping error as shown in Fig. 1 in our paper.} baseline methods and easily improves existing methods} (\textit{KISS-ICP} vs. \textit{KISS-ICP+DM2}).
% We did not include (1) \textit{Fast-LIVO}, because it requires IMU and images which makes the comparisons not ``apple to apple'' for the pure LiDAR mapping task considered in this paper, and (2) \textit{PWCLO-Net}, because the pre-trained model does not converge on the large trajectories.
% % The quantitative results reported in \cref{tab:kitti_ate} \textbf{reinforce our findings that \textit{DM2} significantly outperforms baseline methods} and can be integrated into existing methods (see comparison of \textit{KISS-ICP} and \textit{KISS-ICP+DM2}).
% % the prior works and improves the mapping result of KISS-ICP, especially in terms of translation ATE. 
% % the pre-trained PWCLO-Net model does not converge on the test trajectories. %\ld{Can we add PWCLO-Net to the table in which we indicate it does not converge.}
% We stress that, as expected, pairwise registration methods (e.g., HRegNet and GeoTransformer) suffer from larger mapping errors on large-scale data due to the lack of optimization (e.g. bundle adjustment in SfM) over the inevitable drift. DM2 addresses this issue by design (although it needs either longer runtime or heavier computation).
% % We think it is not proper to directly compare these methods with DM2.


% \cref{fig:training_curve} compares \textit{DM2} with \textit{DM} in detail, where the latter has limited improvement over \textit{ICP} (black dotted line), and both fail on larger scale trajectories. This is why we did not include DM in the original submission.
% % This is because \textit{DM} can only refine local misalignment but not fix drifts on the global scale. 
% The proposed \textit{DM2} is robust on large trajectories and achieves significantly smaller errors than other existing methods.
% %First, \cref{fig:training_curve} demonstrates that the original DeepMapping has almost \emph{no effect} when optimizing ICP on a large-scale scene, because DeepMapping can only refine some local misalignment and is unable to fix any drift error on the global scale.
% \vspace{-2mm}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.47\textwidth]{rebuttal_figs/training_curve.pdf}
%     \vspace{-3mm}
%     \caption{ATE versus training epoch on \textit{KITTI\_0027} 
%     dataset. The error of ICP initialization is also provided for reference.}
%     \label{fig:training_curve}
% \vspace{-2mm}
% \end{figure}

% % \begin{wrapfigure}{l}{0.24\textwidth}
% %   \begin{center}
% %   \vspace{-6mm}
% %     \includegraphics[width=0.26\textwidth]{rebuttal_figs/training_curve.pdf}
% %     \vspace{-6mm}
% %   \caption{\textbf{ATE vs. training epoch} on \textit{KITTI\_0027} 
% %     dataset. The error of ICP initialization is also provided for reference.}
% %     \label{fig:training_curve}
% %   \end{center}
% %   \vspace{-4mm}
% % \end{wrapfigure}

% % \vspace{-2mm}

% % We compare our method with original DeepMapping, HRegNet, GeoTransforme, and we introduce KISS-ICP~\footnote{Vizzo et al., ``KISS-ICP: In defense of point-to-point icp simple, accurate, and robust registration if done the right way,'' IEEE RA-L 2023} instead of Fast-LIVO as state-of-the-art SLAM method, because DeepMapping2 is a LiDAR SLAM which is not fair to compare with LiDAR-Visual-Inertial coupled method like Fast-LIVO. And note that PWCLO-Net cited by Review 1 diverges using the pretrained model.

% % Though we provide these results here, we intentionally avoid comparing pairwise registration methods with DM2 because we think this is not fair for these works. 



% % Second, \cref{tab:kitti_ate} shows that the existing SLAM methods with \emph{bundle adjustment} exceed state-of-the-art pairwise registration methods by a large margin. 

%  % Lastly, we also integrate KISS-ICP with DM2. It can be seen that DM2 improves the mapping result of KISS-ICP, especially in terms of translation ATE.
% % The result shows that the existing SLAM methods with bundle adjustment exceeds SOTA pairwise registration methods by a large margin. 

% % We also highlight that pairwise registration, such as HRegNet and GeoTransformer, has large mapping errors due to the lack of bundle adjustment and optimization components. We think it is not proper to directly compare these methods with DM2.

% \textbf{Reviewers vwoA \& tdMN: Novelty \& effectiveness of DM2's new techniques.
% % New features in DM2.
% } First, the \textit{batch organization} technique is non-trivial and novel as it seamlessly integrates loop closing into DM, while most prior works organize data batches either randomly or temporally. It is not only critical in DM2 but also could inspire new ways of integrating loop closing into deep-learning-based mapping/SLAM methods.
% The second non-trivial novel technique is \textit{the use of pairwise registration} in DM2 and the way we combine it with DM's global registration \textit{via the consistency loss}.
% % Additionally, while we do use existing methods, the overall approach is innovative in that we combine pairwise registration with DM's global registration via consistency loss. 
% We point out that pairwise registration is locally accurate and should not be ignored in DM. Thus we designed the consistency loss to help global registration on large-scale datasets. 

% Note that the consistency loss is NOT ``almost invalid'': the benefit of the two techniques are best revealed when used together than separately (comparing row 2 to 5, not 1 to 3 in Tab. 3). Also, what's important is ``where'' not ``when'' it converges: only DM2 gets to the lowest ATE (\cref{fig:training_curve}).
% % Combining both techniques in the proposed method offers the best mapping results.

% % First, the batch organization is a novel, nontrivial technical step that wasn't included in earlier relevant approaches. Loop closure is implicitly included in the batch organization in the deep learning pipeline.%, which is something previous approaches have not done. By introducing this novel technique, DM2 would automatically include bundle adjustment. 

% % Additionally, self-supervised local-to-global point consistency is another novel technical advancement that has not yet been proposed. Although pairwise registration(ICP) in consistency loss is a known method, combining it in consistency loss is not straightforward because it is based on our observation that pairwise registration has fairly accurate local point cloud registration and can help DM2's global registration on large-scale datasets based on local-to-global consistency. 

% % \cref{fig:training_curve} shows both batch organization and consistency loss cannot work alone. However, batch organization and consistency loss combined with DeepMapping would provide a better mapping result compared with other ablation studies.

% % \xh{@Chao, You need to mention the other two paper mentioned by Reviewer oReC} \xh{Visual odometry vs V-SLAM}
% % Moreover, our method would enhance the KISS-ICP's mapping result.

% % \textbf{Individual Concern}

% % \textbf{Reviewer oReC: Compare with DeepMapping.}
% %  \cref{fig:training_curve} demonstrates that the original DeepMapping has limited capability when optimizing ICP on a large-scale scene. The improvement is almost hard to notice because DeepMapping can only refine some local misalignment and is unable to fix any drift error on the global scale. %Despite its faster convergence, it does not converge to an optimal state, which is meaningless in real applications. \xh{Need Rephrase}
%  % provide any meaningful optimization in large-scale environment.

% % Furthermore,  Figure xxxx on KITTI does not demostrate the optimization capability because the KITTI scene is simple. Thus we update Figure 8 on NCLT dataset.
% \textbf{Reviewers vwoA \& tdMN:  Generalization and runtime cost}. 
% % As stated in the related work section, our work 
% DM2 follows the train-as-optimization LiDAR SLAM framework, so the question of generalization ability is less relevant, not to mention the M-Net and L-Net are still useful as occupancy net and posenet just like in DM. 

% % Furthermore, this train-as-optimization category is adaptive for post map processing tasks. These tasks can be completed offline. 
% Furthermore, the runtime cost in mapping is not the top priority unlike in real-time SLAM: a large-scale mapping algorithm that reduces mapping error significantly is still useful even if it was offline. Moreover, we had acknowledged this limitation and discussed a DDP-based parallel training improvement that has advantages at large scales.

% \vspace{+1mm}

% \textbf{Reviewer oReC: More KITTI sequences.} DM2 still performs better in two shorter KITTI sequences (\cref{tab:kitti_ate}). Note, other much shorter sequences are less informative for benchmarking since even ICP could get good results.
% % In both KITTI sequences, we reach the same conclusion: DM2 performs better than other baselines.
% % are so simple that they can achieve a reasonable mapping result, making it difficult to demonstrate DM2's optimization capabilities. 

% %The quality of the predicted trajectory is measured by absolute trajectory error (ATE) compared with the GPS trajectory. Results on two trajectories are listed. ``T-ATE" means translation ATE (m) ``R-ATE" means rotation ATE (deg). The last two rows are our results.
% % \vspace{-2mm}
% \begin{table}[t]    \caption{\textbf{Additional results on the KITTI dataset.}} 
% \vspace{-2mm}
%     \label{tab:kitti_ate}
%     \centering
%     \resizebox{0.85\linewidth}{!}{%
%     \begin{tabular}{@{}lcccc@{}}
%         \toprule
%         \multirow{2}{*}{\textbf{More baseline}} & \multicolumn{2}{c}{\textbf{Drive\_0018}} & \multicolumn{2}{c}{\textbf{Drive\_0027}} \\
%         & \textbf{T-ATE (m)}$\downarrow$ & \textbf{R-ATE ($^{\circ}$)}$\downarrow$ & \textbf{T-ATE (m)}$\downarrow$ & \textbf{R-ATE ($^{\circ}$)}$\downarrow$ \\
%         \midrule
%         HRegNet & 30.61 & 94.90 & 45.49 & 85.36 \\
%         GeoTransformer & 4.03 & 3.02 & 10.15 & 15.34 \\
%         % PWCLO-Net~\cite{wang2021pwclo} &  &  &  &  \\
%         ICP+DM & 3.42 & 1.66 & 3.39 & 2.70 \\
%         KISS-ICP & 2.10 & 0.68 & 6.25 & 1.21 \\
%         \midrule
%         ICP+\textbf{DM2} & 1.81 & 0.72 & \textbf{2.29} & 1.57 \\
%         KISS-ICP+\textbf{DM2} & \textbf{1.78} & \textbf{0.68} & 2.30 & \textbf{1.17} \\
%         \bottomrule
%     \end{tabular}
%     }

%     \resizebox{0.85\linewidth}{!}{%
%     \begin{tabular}{@{}lcccc@{}}
%         \toprule
%         \multirow{2}{*}{\textbf{More sequence}} & \multicolumn{2}{c}{\textbf{Sequence 02}} & \multicolumn{2}{c}{\textbf{Sequence 08}} \\
%         & \textbf{T-ATE (m)}$\downarrow$ & \textbf{R-ATE ($^{\circ}$)}$\downarrow$ & \textbf{T-ATE (m)}$\downarrow$ & \textbf{R-ATE ($^{\circ}$)}$\downarrow$ \\
%         \midrule
%         Incremental ICP & 8.06 & 4.57 & 4.38 & 4.46 \\
%         Multiway Registration & 4.96 & 3.37 & 2.40 & 0.90 \\
%         \midrule
%         ICP+\textbf{DM2} & \textbf{2.56} & \textbf{1.31} & \textbf{1.85} & \textbf{0.81} \\
%         \bottomrule
%     \end{tabular}
%     }
% \vspace{-5mm}
% \end{table}
% %KISS-ICP~\cite{vizzo2023kiss}

% \textbf{Reviewer tdMN: Warm start limitation}.
% DM2 is like the deep learning version of ``bundle adjustment (BA)'' for LiDAR mapping. And the warm start is like the front-end initialization in SfM before BA. Just like that BA in SfM is affected by the initial solution's quality, it is not surprising that DM2 is affected by warm start quality. We actually consider this an advantage more than a limitation as DM2 can be seamlessly integrated into any mapping front-end and always leads to improvement without manual tuning.
% % DM trains the model in a single batch for small-scale environments, allowing for the creation of accurate LiDAR maps without the need for a warm start. In contrast, if no warm-start is used in a large-scale setting, the network will likely enter a local minimum state. Therefore, we do not overclaim and refer to our method as a LiDAR map optimization method rather than a LiDAR mapping method.

% \textbf{Reviewer tdMN: Visualization}.
% The Nebula dataset is large, and due to the space limit here, we will provide larger views of Fig.~7 and the error heat map in our camera-ready paper. We do not think this reduces our contribution.
% % Additionally, Reviewer tdMN's criticism of the projected consistency loss is invalid. On the other hand, we will take into account the remarks regarding Reviewer oReC: Slow covergence in DeepMapping and update Figure 8 and Table 3 accordingly.

% % The trajectory of Nebula dataset is 590.85 meter long and contains 37,949 LiDAR scans in total.  *******

% % \begin{table}[t]    \caption{\textbf{Additional results on KITTI odometry dataset.}} 
% % \vspace{-2mm}
% %     \label{tab:kitti_ate}
% %     \centering
% %     \resizebox{0.85\linewidth}{!}{%
% %     \begin{tabular}{@{}lcccc@{}}
% %         \toprule
% %         \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Sequence 02}} & \multicolumn{2}{c}{\textbf{Sequence 08}} \\
% %         & \textbf{T-ATE (m)}$\downarrow$ & \textbf{R-ATE ($^{\circ}$)}$\downarrow$ & \textbf{T-ATE (m)}$\downarrow$ & \textbf{R-ATE ($^{\circ}$)}$\downarrow$ \\
% %         \midrule
% %         Incremental ICP & 8.06 & 4.57 & 4.38 & 4.46 \\
% %         Multiway Registration & 4.96 & 3.37 & 2.40 & 0.90 \\
% %         \midrule
% %         ICP+\textbf{DM2} & 2.56 & 1.31 & 1.85 & 0.81 \\
% %         \bottomrule
% %     \end{tabular}
% %     }
% % \vspace{-4mm}
% % \end{table}




% % {\small
% % \balance
% % \bibliographystyle{IEEEtran}
% % \bibliography{egbib}
% % }

% \end{document}

